vq-wav2vec: Self-Supervised Learning of Discrete Speech Representations

We propose vq-wav2vec to learn discrete representations of audio segments through a wav2vec-style self-supervised context prediction task. The algorithm uses either a gumbel softmax or online k-means clustering to quantize the dense representations. Discretization enables the direct application of algorithms from the NLP community which require discrete inputs. Experiments show that BERT pre-training achieves a new state of the art on TIMIT phoneme classification and WSJ speech recognition.

==> fig/experiment-overview.tex <==
\tikzset{%
    feature/.style={draw=none, fill=blue!20, minimum size=0.5cm,text width=2cm,scale=0.9},
    eval/.style={draw=none, fill=green!20, minimum size=0.5cm,text width=2cm,scale=0.9},
    data/.style={draw=none, fill=red!20, minimum size=0.5cm,text width=2cm,scale=0.9}
}
\begin{figure}
    \center
    \begin{tikzpicture}
        \node [feature] (wave) at (0,0) {Waveform};
        \node [feature,right = 3 of wave] (tokens)  {Quantized tokens};
        \node [feature,below right = 1.0 and 0.2 of wave] (densetokens)  {dense\\features};
        \node [feature,right = 1.5 of tokens] (bert)  {Dense BERT features};
        
        \node [data, above = .5 of tokens] (data1) {Libri100/\\Libri960};
        \node [data, above = .5 of bert] (data2) {Libri960/\\LibriVox};
        
        \node [eval,below = .5 of densetokens] (base4) {wav2vec performance};
        \node [eval,below = .5 of wave] (base1) {log-mel Baseline};
        \node [eval,below = .5 of tokens] (base2) {vq-wav2vec Baseline};
        \node [eval,below = .5 of bert] (base3) {BERT performance};
        
        \draw [->] (wave) to node[above] {vq-wav2vec} (tokens);
        \draw [->] (wave) to (wave -| densetokens) to node[right] {wav2vec} (densetokens);
        \draw [->] (tokens) to node[above] {RoBERTa} (bert);
        
        \draw [->] (data1) to (tokens);
        \draw [->] (data2) to (bert);
        
        \draw [->] (wave) to (base1);
        \draw [->] (tokens) to (base2);
        \draw [->] (bert) to (base3);
        \draw [->] (densetokens) to (base4);
        
    \end{tikzpicture}
    \caption{%
        Training setup overview with different measurement points for downstream performance.
        Based on different data representations (blue), we take unlabeled auxilary datasets (red) to derive new feature representation (also blue) with different self-supervised algorithms (arrows).
        Finally, we measure downstream performance on TIMIT and WSJ using \wavtoletter{} (green).
    }
    \label{fig:experiment-overview}
\end{figure}

==> fig/model-overview.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
  \newcommand{\nodedist}{2}
  \newcommand{\charsep}{0.25}
  \newcommand{\charoff}{1.35}
  \newcommand{\depth}{3}
%  \newcounter{totalchar}

  \node [inner sep=0pt, rotate=90] at (-.5*\nodedist,0) {\includegraphics[width=5em, height = 4em]{fig/waveform.pdf}};

  \node [encoder,fill=accent2] (w2v) at (\nodedist*0,0) {};
  \node [encoder,fill=gray!30] (bert) at (\nodedist*1,0) {};
  \node [encoder,fill=accent1] (am) at (\nodedist*2,0) {};
  \node [encoder,fill=gray!30] (dec) at (\nodedist*3,0) {};

  %
  \node [above = .5 of w2v.west] {vq-wav2vec};
  \node [above = .5 of bert.west] {BERT};
  \node [above = .5 of am.west] {AM};
  \node [above = .5 of dec.west] {LM};
  
  \foreach \name in {w2v,bert,dec} {
      \coordinate [below = 0.3 of \name] (\name_arc);
      \draw[thick, <-] (\name_arc) arc (120:420:0.3*\nodedist);
  }
  %\node [below = 0 of w2v_arc] {Self-Sup};
  
  \coordinate [below = 0.3 of dec] (dec_arc);
  \draw[thick, <-] (dec_arc) arc (120:420:0.3*\nodedist);
  %\node [below = 0 of dec_arc] {Self-Sup};
  
  %\draw[thick, ->] (dec.east) arc (120:420:0.3*\nodedist);
  
  %\draw[->, thick] (w2v.east) to [out=-130, in=180] ++(0,-1)  to  [out=0,in=-60] (w2v.east);

  \draw [->, line width = 4pt, draw = FAIRdark!20] (w2v) to (bert);
  \draw[->, line width = 4pt, draw = FAIRdark!20] (bert) to (am);
  \draw[->, line width = 4pt, draw = FAIRdark!20] (am) to (dec);

  %
  \tikzmath{int \total; \total=0;}
  \foreach \c/\r [count=\x from 0] in {t/2,h/1,e/2,{ }/1,c/1,a/3,t/1} {
    % draw the emission

    \foreach \y in {1,...,\r} {
      %\node at (\nodedist*1.5, -\arabic{totalchar}*\charsep + \charoff) {\small \c};
      \stepcounter{totalchar};
    }
    % draw the decoded char
    \node at (\nodedist*3.5, -\x*\charsep*1.5 + \charoff) {\c};
  }

\end{tikzpicture}
\caption{%
    The full training setup includes the vq-wav2vec quantizer, a BERT language model in front of the acoustic model, and another language model for decoding after the acoustic model, all of which are trained with self-supervised objectives.
    Only the acoustic model is trained with a supervised loss function.
}
\label{fig:model-overview}
\end{figure}

==> fig/quantizer-pruned.tex <==
\newcommand{\dimscale}{7.5pt}
\newcommand{\skipdist}{.5}
\newcommand{\hskipdist}{1.5*\skipdist}
\newcommand{\vskipdist}{1.5*\skipdist}

\newcommand{\dimd}{8}
\newcommand{\dimdG}{4}
\newcommand{\dimG}{1
}
\newcommand{\dimC}{5}

\newcommand{\bgcolor}{gray!10}

\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)


\newcommand{\drawmatrix}[5]{%
    \node [rectangle,
        rounded corners,
    fill=#5, minimum height = #2*\dimscale, minimum width = #3*\dimscale, #4] (#1) {};
    
    %\coordinate [#4] (#1);
    \coordinate (#1_anchor) at ($(#1) -(0.5*#3*\dimscale,0.5*#2*\dimscale)$);

    \draw[%
        step=\dimscale,
        \bgcolor,
        thick,
        shift={(#1_anchor)},
        line cap=round,
        ] (0,0) grid +(#3*\dimscale,#2*\dimscale);

    %\foreach \x in {1,...,#3} {
    %    \foreach \y in {1,...,#4} {
    %        \node [rectangle, minimum height = \dimscale, minimum width = \dimscale, draw=black] at (0,0) {};
    %    }
    %}

    %\coordinate [#4] (#1);
    %\draw[step=0.5*\dimscale, #5] ($(#1) +(-#3*\dimscale,-#2*\dimscale)$) grid +(2*#3*\dimscale,2*#2*\dimscale);

}

\newcommand{\drawtensor}[6] {
    %\node [rectangle, fill=#5, minimum height = #2*\dimscale, minimum width = #3*\dimscale, #4] (#1) {};
    \coordinate [#5] (#1_pre);
    \coordinate (#1) at ($(#1_pre) - (0,1.5*\dimscale)$);
    
    \coordinate (#1_anchor) at ($(#1_pre) -(0.75*#3*\dimscale,0.5*#2*\dimscale)$);

    \draw[%
        step=\dimscale,
        \bgcolor,
        thick,
        fill=#6,
        shift={(#1_anchor)},
        line cap=round,,
        ] (0,0) grid +(#3*\dimscale,#2*\dimscale) rectangle (0,0);

    % right side
    \coordinate (#1_anchor_right) at ($(#1_anchor) +(#3*\dimscale,0)$);
    \draw[%
        step=\dimscale,
        yslant=1,
        xscale=0.5,
        \bgcolor,
        fill=#6,
        thick,
        shift={(#1_anchor_right)},
        line cap=round,%
    ] (0,0) grid +(#4*\dimscale,#2*\dimscale) rectangle (0,0);

    % top side
    \coordinate (#1_anchor_top) at ($(#1_anchor) +(0,#2*\dimscale)$);
    \draw[%
        step=\dimscale,
        xslant=1,
        yscale=0.5,
        \bgcolor,
        fill=#6,
        thick,
        shift={(#1_anchor_top)},
        line cap=round,%
    ] (0,0) grid +(#3*\dimscale,#4*\dimscale) rectangle (0,0); 
    
    \coordinate (#1_anchor_north) at ($(#1_anchor_top) +(#3*\dimscale,.5*#4*\dimscale)$);

}

\begin{figure}
\centering

    \begin{minipage}{0.48\textwidth}
\centering
    \resizebox{\textwidth}{!}{

        \begin{tikzpicture}[scale = 1]

        % inputs


        % coordinate definitions
        \coordinate (origin) at (0,0);
        \coordinate (lower) at (0, -2);

        % d x 1
        \drawmatrix{ze}{\dimd}{1}{right = 0 of origin}{\colorze}
        \drawmatrix{logits}{1}{\dimC}{right = 1 of ze}{\colorze}
        \drawmatrix{probs}{1}{\dimC}{above = .2 of logits}{\colorze}
        \drawmatrix{onehot}{1}{\dimC}{above = .2 of probs}{\colorze}
        
        %\node [above = .5 of zee] (gumbel) {$g \sim \Gumbel(0,1)$};
        %\draw[->] (gumbel) to (ze.west);

        %\drawmatrix{i}{\dimG}{1}{below right = \hskipdist of zee_gumbel}{\colori}
        
        %\node [] (dot) at ($(zee_gumbel.east)!0.5!(zqq.west)$) {$\times$};
        \drawmatrix{e}{\dimd}{\dimC}{above = \vskipdist of onehot}{\colore}
        %\draw[->] (zee_gumbel) to (dot) to (zqq);
        %\draw[->] (e) to (dot);
        
        \drawmatrix{zq}{\dimd}{1}{right = \hskipdist of probs}{\colorzq}
        

        \foreach \f/\t in {ze/logits, logits/probs, probs/onehot}
            \draw[->] (\f) to (\t);


        % annotations below
        \node[above left=1.3 of e] {$\e$};
        
        \begin{pgfonlayer}{bg}
            \node[rectangle,
                fit = {(ze) (logits) (e) (i) (zqq) (zq)},
                inner sep = 12pt,
                draw=gray,
                fill=gray!10
            ] (box) {};
        \end{pgfonlayer}
        
        \node[above = 0.25 of box.north west, anchor = west] {A. Gumbel VQ-wav2vec};

        \end{tikzpicture}
    }

        
    \end{minipage}\quad
    \begin{minipage}{0.48\textwidth}
\centering
    \resizebox{\textwidth}{!}{

        \begin{tikzpicture}[scale = 1]

        % inputs

        % coordinate definitions
        \coordinate (origin) at (0,0);
        \coordinate (lower) at (0, -2);

        % d x 1
        \drawmatrix{ze}{\dimd}{1}{right = 0 of origin}{\colorze}
        \drawmatrix{zee}{\dimG}{\dimdG}{right = \hskipdist of ze}{\colorzee}
        \drawmatrix{d}{\dimG}{\dimC}{right = \hskipdist of zee}{\colord}

        \drawtensor{e}{\dimG}{\dimC}{\dimdG}{above = \vskipdist of d}{\colore}
        \drawmatrix{i}{\dimG}{1}{right = \hskipdist of d}{\colori}
        \drawmatrix{zqq}{\dimG}{\dimdG}{right = \hskipdist of i}{\colorzqq}
        \drawmatrix{zq}{\dimd}{1}{right = \hskipdist of zqq}{\colorzq}

        \foreach \f/\t in {ze/zee, zee/d, e/d, d/i, zqq/zq}
            \draw[->] (\f) to (\t);

        \node[circle, above = 0.5 of i] (index) {$\times$};
        \draw[->] (i) to (index);
        \draw[->] (e_anchor_right) to (index);
        \draw[->] (index) to (zqq |- e) to (zqq);
        

        % annotations
        \foreach \name/\annot/\symb in {%
            ze/$\R^d$/$\ze$,
            zee/$\R^{G \times d/G}$/$\ze'$,
            d/$\R^{G \times C}$/$\|\zq' - \e \|_2^2$,
            i/$[C]^G$/$\idx$,
            zqq/$\R^{G \times d/G}$/$\zq'$,
            zq/$\R^{d}$/$\zq$
            }{
            %\node [below = .1 of \name] {\small \annot};
            \node [below = .1 of \name] {\small \symb};
        }
        \node[above left=1.3 of e] {$\e$};
        
        \begin{pgfonlayer}{bg}
            \node[rectangle,
                fit = {(ze) (zee) (e) (i) (zqq) (zq)},
                draw=gray,
                inner sep = 12pt,
                fill=gray!10
            ] (box) {};
        \end{pgfonlayer}
        
        \node[above = 0.25 of box.north west, anchor = west] {B. k-means VQ-wav2vec};
        
        \draw[->,dashed,rounded corners] (zqq.south west)
            to +(0,-\vskipdist)
            to ($(zee.south east) +(0,-1*\vskipdist)$)
            to (zee.south east);

        \end{tikzpicture}
    }

    \end{minipage}
    \caption{\textbf{A.} Gumbel Softmax vector quantization module.
    The dot product between Gumbel probabilities and the codebook embedding tensor ($\times$) is evaluated by one-hot coding in the forward pass, and used exactly during the backward pass.
    %
    \textbf{B.} K-means vector quantization module.
    Indices are selected by evaluating the distance matrix between embeddings and features.
    }

\end{figure}

==> fig/quantizer.tex <==
\newcommand{\dimscale}{7.5pt}
\newcommand{\skipdist}{.5}
\newcommand{\hskipdist}{1.5*\skipdist}
\newcommand{\vskipdist}{1.5*\skipdist}

\newcommand{\dimd}{8}
\newcommand{\dimdG}{4}
\newcommand{\dimG}{1
}
\newcommand{\dimC}{5}

\newcommand{\bgcolor}{gray!10}

\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)


\newcommand{\drawmatrix}[5]{%
    \node [rectangle, fill=#5, minimum height = #2*\dimscale, minimum width = #3*\dimscale, #4] (#1) {};
    
    %\coordinate [#4] (#1);
    \coordinate (#1_anchor) at ($(#1) -(0.5*#3*\dimscale,0.5*#2*\dimscale)$);

    \draw[%
        step=\dimscale,
        \bgcolor,
        thick,
        shift={(#1_anchor)},
        line cap=round,
        ] (0,0) grid +(#3*\dimscale,#2*\dimscale);

    %\foreach \x in {1,...,#3} {
    %    \foreach \y in {1,...,#4} {
    %        \node [rectangle, minimum height = \dimscale, minimum width = \dimscale, draw=black] at (0,0) {};
    %    }
    %}

    %\coordinate [#4] (#1);
    %\draw[step=0.5*\dimscale, #5] ($(#1) +(-#3*\dimscale,-#2*\dimscale)$) grid +(2*#3*\dimscale,2*#2*\dimscale);

}

\newcommand{\drawtensor}[6] {
    %\node [rectangle, fill=#5, minimum height = #2*\dimscale, minimum width = #3*\dimscale, #4] (#1) {};
    \coordinate [#5] (#1_pre);
    \coordinate (#1) at ($(#1_pre) - (0,1.5*\dimscale)$);
    
    \coordinate (#1_anchor) at ($(#1_pre) -(0.75*#3*\dimscale,0.5*#2*\dimscale)$);

    \draw[%
        step=\dimscale,
        \bgcolor,
        thick,
        fill=#6,
        shift={(#1_anchor)},
        line cap=round,,
        ] (0,0) grid +(#3*\dimscale,#2*\dimscale) rectangle (0,0);

    % right side
    \coordinate (#1_anchor_right) at ($(#1_anchor) +(#3*\dimscale,0)$);
    \draw[%
        step=\dimscale,
        yslant=1,
        xscale=0.5,
        \bgcolor,
        fill=#6,
        thick,
        shift={(#1_anchor_right)},
        line cap=round,%
    ] (0,0) grid +(#4*\dimscale,#2*\dimscale) rectangle (0,0);

    % top side
    \coordinate (#1_anchor_top) at ($(#1_anchor) +(0,#2*\dimscale)$);
    \draw[%
        step=\dimscale,
        xslant=1,
        yscale=0.5,
        \bgcolor,
        fill=#6,
        thick,
        shift={(#1_anchor_top)},
        line cap=round,%
    ] (0,0) grid +(#3*\dimscale,#4*\dimscale) rectangle (0,0); 
    
    \coordinate (#1_anchor_north) at ($(#1_anchor_top) +(#3*\dimscale,.5*#4*\dimscale)$);

}

\begin{figure}
\centering

    \begin{minipage}{0.48\textwidth}
\centering
    \resizebox{\textwidth}{!}{

        \begin{tikzpicture}[scale = 1]

        % inputs


        % coordinate definitions
        \coordinate (origin) at (0,0);
        \coordinate (lower) at (0, -2);
        

        % d x 1
        \drawmatrix{ze}{\dimd}{1}{right = 0 of origin}{\colorze}
        \drawmatrix{zee}{\dimG}{\dimdG}{right = \hskipdist of ze}{\colorzee}
        \drawmatrix{zee_gumbel}{\dimG}{\dimC}{right = \hskipdist of zee}{\colorgumbel}
        
        \node [above = .5 of zee] (gumbel) {$g \sim \Gumbel(0,1)$};
        \draw[->] (gumbel) to (zee_gumbel.west);

        \drawmatrix{i}{\dimG}{1}{below right = \hskipdist of zee_gumbel}{\colori}
        \drawmatrix{zqq}{\dimG}{\dimdG}{right = \hskipdist of zee_gumbel}{\colorzqq}
        \drawmatrix{zq}{\dimd}{1}{right = \hskipdist of zqq}{\colorzq}
        
        \node [] (dot) at ($(zee_gumbel.east)!0.5!(zqq.west)$) {$\times$};
        \drawtensor{e}{\dimG}{\dimC}{\dimdG}{above = \vskipdist of dot}{\colore}
        \draw[->] (zee_gumbel) to (dot) to (zqq);
        \draw[->] (e) to (dot);
        

        \foreach \f/\t in {ze/zee, zee/zee_gumbel, zee_gumbel/i, zqq/zq}
            \draw[->] (\f) to (\t);


        % annotations below
        \foreach \name/\annot/\symb in {%
            zee/$\R^{G \times d/G}$/$\ze'$,
            zee_gumbel/$\R^{G \times d/G}$/$\mathbf{p}$,
            zqq/$\R^{G \times d/G}$/$\zq'$,
            zq/$\R^{d}$/$\zq$,
            ze/$\R^d$/$\ze$
            }{
            \node [below = .1 of \name] {\small \symb};
        }
        \foreach \name/\annot/\symb in {%
            i/$[C]^G$/$\idx$
            }{%
            \node [left = .1 of \name] {\small \symb};
        }
        \node[above left=1.3 of e] {$\e$};
        
        \begin{pgfonlayer}{bg}
            \node[rectangle,
                fit = {(ze) (zee) (e) (i) (zqq) (zq)},
                inner sep = 12pt,
                draw=gray,
                fill=gray!10
            ] (box) {};
        \end{pgfonlayer}
        
        \node[above = 0.25 of box.north west, anchor = west] {A. Gumbel VQ-wav2vec};

        \end{tikzpicture}
    }

        
    \end{minipage}\quad
    \begin{minipage}{0.48\textwidth}
\centering
    \resizebox{\textwidth}{!}{

        \begin{tikzpicture}[scale = 1]

        % inputs

        % coordinate definitions
        \coordinate (origin) at (0,0);
        \coordinate (lower) at (0, -2);

        % d x 1
        \drawmatrix{ze}{\dimd}{1}{right = 0 of origin}{\colorze}
        \drawmatrix{zee}{\dimG}{\dimdG}{right = \hskipdist of ze}{\colorzee}
        \drawmatrix{d}{\dimG}{\dimC}{right = \hskipdist of zee}{\colord}

        \drawtensor{e}{\dimG}{\dimC}{\dimdG}{above = \vskipdist of d}{\colore}
        \drawmatrix{i}{\dimG}{1}{right = \hskipdist of d}{\colori}
        \drawmatrix{zqq}{\dimG}{\dimdG}{right = \hskipdist of i}{\colorzqq}
        \drawmatrix{zq}{\dimd}{1}{right = \hskipdist of zqq}{\colorzq}

        \foreach \f/\t in {ze/zee, zee/d, e/d, d/i, zqq/zq}
            \draw[->] (\f) to (\t);

        \node[circle, above = 0.5 of i] (index) {$\times$};
        \draw[->] (i) to (index);
        \draw[->] (e_anchor_right) to (index);
        \draw[->] (index) to (zqq |- e) to (zqq);
        

        % annotations
        \foreach \name/\annot/\symb in {%
            ze/$\R^d$/$\ze$,
            zee/$\R^{G \times d/G}$/$\ze'$,
            d/$\R^{G \times C}$/$\|\zq' - \e \|_2^2$,
            i/$[C]^G$/$\idx$,
            zqq/$\R^{G \times d/G}$/$\zq'$,
            zq/$\R^{d}$/$\zq$
            }{
            %\node [below = .1 of \name] {\small \annot};
            \node [below = .1 of \name] {\small \symb};
        }
        \node[above left=1.3 of e] {$\e$};
        
        \begin{pgfonlayer}{bg}
            \node[rectangle,
                fit = {(ze) (zee) (e) (i) (zqq) (zq)},
                draw=gray,
                inner sep = 12pt,
                fill=gray!10
            ] (box) {};
        \end{pgfonlayer}
        
        \node[above = 0.25 of box.north west, anchor = west] {B. k-means VQ-wav2vec};
        
        \draw[->,dashed,rounded corners] (zqq.south west)
            to +(0,-\vskipdist)
            to ($(zee.south east) +(0,-1*\vskipdist)$)
            to (zee.south east);

        \end{tikzpicture}
    }

    \end{minipage}
    \caption{\textbf{A.} Gumbel Softmax vector quantization module.
    The dot product between Gumbel probabilities and the codebook embedding tensor ($\times$) is evaluated by one-hot coding in the forward pass, and used exactly during the backward pass.
    %
    \textbf{B.} K-means vector quantization module.
    Indices are selected by evaluating the distance matrix between embeddings and features.
    \stes{TODO replace by new figure}
    }

\end{figure}
